Secure Inter-domain Routing and Forwarding via Verifiable Forwarding Commitments

The Internet inter-domain routing system is vulnerable. On the control plane, the de facto Border Gateway Protocol (BGP) does not have built-in mechanisms to authenticate routing announcements, so an adversary can announce virtually arbitrary paths to hijack network traffic; on the data plane, it is difficult to ensure that actual forwarding path complies with the control plane decisions. The community has proposed significant research to secure the routing system. Yet, existing secure BGP protocols (e.g., BGPsec) are not incrementally deployable, and existing path authorization protocols are not compatible with the current Internet routing infrastructure. In this paper, we propose FC-BGP, the first secure Internet inter-domain routing system that can simultaneously authenticate BGP announcements and validate data plane forwarding in an efficient and incrementally-deployable manner. FC-BGP is built upon a novel primitive, name Forwarding Commitment, to certify an AS's routing intent on its directly connected hops. We analyze the security benefits of FC-BGP in the Internet at different deployment rates. Further, we implement a prototype of FC-BGP and extensively evaluate it over a large-scale overlay network with 100 virtual machines deployed globally. The results demonstrate that FC-BGP saves roughly 55% of the overhead required to validate BGP announcements compared with BGPsec, and meanwhile FC-BGP introduces a small overhead for building a globally-consistent view on the desirable forwarding paths.

==> analysis.tex <==
\section{Analysis}
\label{sec:analysis}

% In this section, we discuss the security benefits and deployability of \sys.

\subsection{Security Benefits}
\label{sub:SecurityBenefits}



\begin{figure}[t]    
\centering
\includegraphics[width=0.95\columnwidth]{picture/securitybenefits-part1-0505.pdf}
\caption{BGP path protection under different deployment rates.}
\label{bgppath1}
\end{figure}

\begin{figure}[t]    
\centering
\includegraphics[width=0.98\columnwidth]{picture/bpgsec-FC-path.pdf}
\caption{BGP path protection of \sys and BGPsec for different path lengths at 5\% deployment rate.}
\label{bgppath2}
\end{figure}

We reconstructed the AS relationships, ownership of prefixes, and the monitored BGP paths using the dataset released by CAIDA in January 2023\footnote{https://publicdata.caida.org/datasets/routing/routeviews-prefix2as/} \footnote{https://publicdata.caida.org/datasets/as-relationships/serial-1/}. 
In total, we measured $74859$ ASes, $380191619$ BGP paths, and $963369$ prefixes. We analyze the extent to which the control plane paths, data plane forwarding paths, and source addresses are protected given different rates of deploying \sys. % Given a deployment rate, we simulate 
% Without loss of generality, we start 

% Since each AS has a different deployment value, we simulated the deployment of \sys in descending order of the number of AS's neighbors, and analyzed the protection of BGP paths, forwarding paths, and source addresses by \sys with different deployment rates.


\subsubsection{BGP Path Protection} 

For the convenience of analysis, we assume that all ASes have an equal probability of being compromised and acting arbitrarily. 
%The more hops that can be validated on a BGP path, the higher the reliability of the path. 
When AS $A$ deploys \sys, the hops originated from $A$ are secured since malicious ASes cannot forge \fcs on behalf of $A$. 
% as the source are considered to be protected. Because no malicious AS can spoof the forwarding commitment of $A$. 
Given an $N$-hop path $p$ with $M$ ASes deployed \sys $(M \leq N)$, we define its protection rate $R_\textsf{BGPpath}$ as $\frac{M}{N}$. As $M$ increases, $R_\textsf{BGPpath}$ increases, and the path $P$ is fully protected if $R_\textsf{BGPpath}=1$. 
Given a set path $\mathbf{S}$ with $K$ BGP paths, we define $\Bar{R}$ as the BGP path protection rate, and define $R_{\textsf{full}}$ as the full path protection ratio. 

\begin{equation}
   \Bar{R} = \frac{R_\textsf{BGPpath}(P)}{K} , \{P \vert P \in \mathbf{P}\}
\label{equ:r}
\end{equation}

\begin{equation}
   R_{\textsf{full}} = \frac{\left| P \right|}{K} ~~\text{where}~~ \{ P \in \mathbf{P} ~~\text{and}~~ R_\textsf{BGPpath}(P) = 1\}
\label{equ:fp}
\end{equation}


We report the $\Bar{P}$ and $R_{\textsf{full}}$ under different deployment rates in Figure~\ref{bgppath1}. We sort the ASes in descending order based on their degrees (\ie the number of neighbors). Given a deployment rate $r\%$, we select the first $r\%$ ASes to deploy \sys. The results show that with only a small percentage of ASes deployed, \sys can achieve significant BGP path protections. 
For instance, when only deploying \sys on the first 1\% ASes, the average protection rate of all monitored BGP paths reaches 83.26\%, and 55.47\% of these paths are fully protected; when the deployment rate reaches 5\%, the two metrics jump to 94.68\% and 81.91\%, respectively.
This indicates that with a only small fraction of deployment, \sys can secure the vast majority of BGP paths in the Internet. 
% Considering that BGPsec becomes effective only if the complete path is protected, \sys provides higher path protection than BGPsec in partial deployments. 


In Figure~\ref{bgppath2}, we fix the deployment rate as 5\%, and plot the path protection rate of \sys and BGPsec for different path lengths. The results show that as the path length increases, the path protection rate of BGPsec decreases significantly. This is expected because BGPsec is effective only if all on-path ASes are upgraded. 
%while the decrease of \sys is smaller and more flat. 
% For example, when the path length increases from 1 to 7, the path protection rate of \sys decreases by about 20.73\%, while BGPsec decreases by about 91.18\%.



% and the results are shown by the two blue lines in Figure~\ref{Sec-Ben}. When we increase the deployment rate to 5\%, a significant security benefit is achieved, 

\subsubsection{Forwarding Path Protection} 

\begin{figure}[t]    
\centering
\includegraphics[width=0.95\columnwidth]{picture/securitybenefits-part2-0502.pdf}
\caption{Forwarding Path Protection under different deployment rates of \sys}
\label{forwardingpath}
\end{figure}


Unlike control plane routing path validation that is primarily based on per-hop \fcs, path forwarding validation must be at the granularity of path. For instance, 
For instance, a BGP path $A{\rightarrow}B{\rightarrow}C{\rightarrow}D$ announced by AS $A$ can derive three different data-plane forwarding paths: $D{\rightarrow}C{\rightarrow}B{\rightarrow}A$, $C{\rightarrow}B{\rightarrow}A$ and $B{\rightarrow}A$. Taking $D{\rightarrow}C{\rightarrow}B{\rightarrow}A$ as an example. Suppose that AS $C$ and $B$ are \sys-aware. If the source AS $D$ is legacy, it will not generate the binding message for traffic $\langle \textsf{src}{:}D,\textsf{dst}{:}A\rangle$. 
As a result, AS $B$ and $C$ will not install filters for traffic $\langle \textsf{src}{:}D,\textsf{dst}{:}A\rangle$, resulting in zero protection for this  forwarding path despite partial deployment at ASes $B$ and $C$. 
We define the metrics similar to Equations~(\ref{equ:r}) and (\ref{equ:fp}) for forwarding path protection, and report evaluation results in Figure~\ref{forwardingpath}. 

%At the initial 1\% deployment, the average protection for all forwarding paths is 51.98\%, and the 44.75\% of them are fully secured; at 5\% deployment, the two metrics are 73.08\% and 67.79\%.  
%As expected, securing forwarding paths requires larger deployment rates. 
% When the deployment rate reaches about 40\%, both the $\Bar{P}$ and the $FP$ can be increased to over 90\%.
% using the two similar metrics as the control plane 


The experimental results show that, \sys achieves significant security benefits with a small number of deployments, and the benefits increase gradually as the deployment rate increases. Specifically, at the initial 1\% deployment, the $\Bar{P}$  51.98\%, and the $P_\textsf{full}$ reaches 44.75\%. When the deployment rate rises to 5\%, the $\Bar{P}$ reaches 73.08\%, and the $P_\textsf{full}$ has reached 67.79\%. When the deployment rate reaches about 40\%, both the $\Bar{P}$ and the $P_\textsf{full}$ can be increased to over 90\%.

% Different from BGP path validation, a single BGP announced path represents multiple data-plane forwarding paths. At the same time, for the forwarding path validation of \sys to take effect for a hop <source $S$, destination D> on path $P$ from $A$ to $B$, both $A$ and $D$ need to be deployed. If $A$ is not deployed, no binding message can be broadcast, and if $D$ is not deployed, no inspection can be performed for traffic from $A$. When A and D both deployed, we refer <$S$,$D$> as a protected hop. For a $N$-hop path $P$ with $M$ protected hops, we defined the protected rate as $M/N$. 

% We analyzed the number of protected hop on each forwarding path for different deployment rates and obtained the $PR_{forwardingpath}$ for each path. Using Equations ~\ref{p} and ~\ref{fp}, we calculated the average forwarding path protection rate $\Bar{P}$ and full forwarding path protection rate $FP$, the results are shown in the two green lines in Figure~\ref{Sec-Ben}. Similar to BGP path validation, for a forwarding path $P$, when on-path nodes are partially deployed, \sys cannot fully protect the security of $P$. However, the higher the deployment rate of on-path nodes, the more reliable $P$ is. When on-path nodes are fully deployed, complete end-to-end path validation can be provided. 

% For a prefix $P$ owned by AS $A$, a single BGP announced path, 
% cannot provide any validation for the traffic from $D$ to $A$, its protection rate is 0\%. When $D$ is deployed, $D{\rightarrow}C$ and $C{\rightarrow}B$ can both provide validation for $D$'s traffic. So the protection rate of about 66\% can be achieved. 




\subsubsection{Source Address Protection} 

We designed two metrics to evaluate the effectiveness of \sys in protecting  source addresses. 
% from both protection scope and security level perspectives. 
One is the protected prefix rate ($PPR$), which is used to evaluate the percentage of prefixes protected by \sys.  %as the deployment rate increases. 
The other metric is \emph{security level} of prefixes ($\Delta SLP$), which is used to assess the incremental changes of prefix security levels as the deployment rate increases. 

% average magnitude of the security benefits of protected prefixes as the deployment rate increases compared to the previous deployment rate.

\begin{figure}[t]    
\centering
\includegraphics[width=0.99\columnwidth]{picture/SAV1.pdf}
\caption{Security Level of Prefix}
\label{SLP}
\end{figure}

\parab{PPR} Suppose that with  deployment rate $d$, the total number of prefixes owned by ASes in \sys ecosystem is $M$, and the number of all prefixes in the entire Internet is $N$. We define the PPR as $M/N$.

\parab{Security Level of Prefix} 
$SLP$ represents the security level of a particular prefix evaluated by all upgraded ASes. For example, as shown in Figure~\ref{SLP}, suppose AS $B$ has $K$ neighbors and we assume that it may receive spoofed traffic from all neighbors with equal probability. When both AS $A$ (owning prefix $P_A$) and AS $B$ (owing prefix $P_B$) deploy \sys, only one of the $K_B$ neighbors of $B$ may receive the binding message $\mathcal{M}_{\textsf{OnPath}}$ for traffic $\langle\textsf{src}{:}P_A,\textsf{dst}{:}P_B\rangle$, 
Thus, AS $B$ is able to detect spoofed traffic forwarded from all remaining $K_B$-1 neighbors. Therefore, 
%for any prefix $P_B$ owned by AS $B$, 
the $SLP$ of prefix $P_A$ assessed from the perspective of $P_B$, under deployment rate $d$, is $SLP_{P_A,P_B}^d=(K_B-1)/K_B$. 
Suppose $S$ is the sets of all prefixes whose owners deploy \sys at deployment rates $d$, then the overall $SLP$ of $P_A$ is obtained by averaging all per-prefix $SLP$, as shown in Equation~(\ref{SLP}). 

\iffalse
\begin{figure}[t]    
\includegraphics[width=0.95\columnwidth]{BGP-Latex/picture/SAV2.pdf}
\caption{Increased Security Level between two deployment rates}
\label{ISPL}
\end{figure}
\fi

\begin{equation}
   SLP_{P_A}^{d} = \frac{{\sum_{p\in S}\frac{K_{p}-1}{K_p}}}{\left|S\right|}
\label{SLP}
\end{equation}


\parab{$\Delta$SLP}
At a given deployment rate, we can obtain an average $SLP$ for all upgraded prefixes. 
Then $\Delta SLP$ represents the incremental change of the two $SLP$ obtained in two different deployment rates. Specifically, the $\Delta SLP$ between two deployment rates $d$ and $d_{pre}$ is defined as 

\begin{equation}
   \Delta SLP_{d,d_{pre}} = \frac{\sum_{p\in S_d}(SLP_{p}^{d}-SLP_{p}^{d_{pre}})}{\left|S_d\right|}, 
\label{PRs}
\end{equation}
where $S_d$ is the set of upgraded prefixes at deployment rate $d$. 

% is the difference between the security level of prefixes ($SLP$) at two different deployment rates. 
% AS $B$ will be able to defend against traffic with spoofed prefix $P$ forwarded at the 
% When both AS $A$ (owning prefix $P_A$) and AS $B$ deploy \sys, AS $A$ will broadcast the binding message corresponding to the selected path with one and only one neighbor of AS $B$. 



%Note that for an AS with a larger number of neighbors $k$, it deploys \sys with a higher $SLP$ evaluation for other prefixes. As shown in Figure~\ref{ISPL}, we consider the state when the deployment rate is $d$, and the state when the deployment rate is $d-pre$ ($d-pre<d$). $S_d$ and $S_{d-pre}$ are the sets of all protected prefixes under the deployment rates $d$ and $d-pre$, respectively.. As the deployment rate increases, ASes with a smaller number of neighbors join the \sys ecosystem. These newly added ASes lower the $SLP$ evaluation of existing prefixes because they have fewer neighbors. However, on the other hand they also significantly improve the $SLP$ evaluation of their own prefixes. For two states with deployment rates of $d$ and $d-pre$, we calculate the $SLP$ difference for each prefix and then average all the differences. We define this average value is $\Delta SLP_{d,d-pre}$, as

% For an AS $A$ with $K$ neighbors, assume that $A$ may receive spoofed traffic from all neighbors with equal probability. %with spoofed source addresses. 
% When both AS $A$ and AS $B$ (which legally owns prefix $P$) deploy \sys, AS $B$ will broadcast the binding message corresponding to the selected path with one and only one neighbor of AS $A$. 
% AS $A$ will be able to defend against traffic with spoofed prefix $P$ forwarded at the remaining $K$-1 neighbors. Therefore, for a deployed AS, its prefixes can be protected within the ecosystem of the \sys. In the case of deployment rate $d$, the total number of prefixes owned by ASes in \sys's ecosystem is $M$, and the number of all prefixes in the entire Internet is $N$. We define the protected prefix rate $PP$ as $M/N$. Meanwhile, for the set $S$ of all deployed ASes and the set $P$ of all legal prefixes owned by $S$, we define the average protection rate of a prefix called $PR_{perfix}^{S}$ as,

% \begin{equation}
%    PR_{perfix}^{S} = \frac{{\sum_{s\in S}\frac{K_{s}-1}{K_s}}}{\left|S\right|}
% \label{PRp}
% \end{equation}

% To analyze the gain in prefix protection rate as the deployment rate increases, we design the following metrics. In experiments with deployment rate of $d$, the set of all deployed nodes is $S_d$, and in experiments with deployment rate of $d$-$pre$ ($d$-$pre<d$), the set of deployed nodes is $S_{d-pre}$. We define the increased prefix protection rate for deployment rate $\Delta PR_{prefix}^{S_d}$ as Equation~\ref{PRs}, representing the average increase in the average protection rate of prefix within \sys's ecosystem from deployment rate $d$ to $d$-$pre$.



% For the convenience of analysis, we assume that for any AS $A$, traffic with its legal prefix as the source is sent to all other ASes with equal probability. For another AS $B$, assuming it has $k$ neighbors, when the route is not changed and there is no source address spoofing, the traffic it observes with $A$ as the source will be forwarded from only one directly connected neighbor (inter-domain single path). Therefore, when both $A$ and $B$ deploy \sys, $B$ will be informed of the correct inbound direction of traffic with $A$ as the source, and traffic from other directions carrying $A$'s legitimate prefix will be considered as source address spoofing.

% If all ASes on the forwarding path from $A$ to $B$ deploy \sys, then $B$ considers $A$'s prefix to be 100\% secure. However, we are limited by the fact that we do not know the actual data-plane forwarding paths of all inter-domain traffic, so there is still the possibility of on-path nodes spoofing source addresses. But for $B$, at least the possibility of spoofing the other $k-1$ incoming directions has been ruled out. Therefore, for $B$, the lower bound of the authenticity of $A$'s prefix at this time is: $(k-1)/k$.

% We take this theoretical lower bound as the security rate of $B$ for the prefix of $A$. We define the prefix protection rate of an AS $A$ to be the average security rate from all other deployed ASes to the prefix of $A$. Since we assume that for any AS $A$, traffic with its legal prefix as the source is sent to all other ASes with equal probability, all prefixes of $A$ have the same protection rate. An undeployed AS has a protection rate of 0\% for its prefix and a security rate of 0\% for other ASes.

\begin{figure}[t]  
\centering
\includegraphics[width=0.95\columnwidth]{picture/securitybenefits-part3.pdf}
\caption{Security Benefits of Source Address Protection}
\label{SLP}
\end{figure}

\parab{Results} 
We report the $PPR$ and $\Delta SLP$ at different deployment rates in Figure~\ref{SLP}. 
% We calculate the $PPR$ at different deployment rates and $\Delta SLP$ as each deployment rate increases, the results are shown as the two red lines in Figure~\ref{Sec-Ben}. 
The results show that the $PPR$ is steadily increasing as the deployment rate increases, from about 18.33\% of prefixes protected at 1\% deployment rate to about 40\% of prefixes protected at 5\% deployment rate. When the deployment rate is further increased to 50\%, more than 80\% of prefixes are protected. 
Meanwhile, $\Delta SLP$ at all deployment rates are strictly positive, indicating that the security levels of prefixes consistently grow. As expected, the marginal increase of $\Delta SLP$ reduces as the deployment rate increases.  
%increases monotonically with the deployment rate, although the increase appears to slow down significantly. 
% The $\Delta SLP$ increases significantly at the beginning of the deployment, with the increase by about 99.75\% as the deployment rate increases from 0\% to 1\%. This is due to the fact that for the first 1\% of AS, the number of neighbors is very high, and when \sys is deployed, the average protection rate of source prefixes can reach a very high level. As the deployment rate increases, the number of neighbors of the AS decreases and the $SLP$ obtained decreases relatively. While the protection rate of the prefixes still maintains a positive increase, the increase rate starts to slow down gradually.

% \subsection{Consensus Correctness}
% We give a brief proof that the our consensus protocol achieve all three goals. Since all RBC instances in our consensus are independent, we only need to analyze the following three goals for one specific RBC instance $\mathcal{R}_i$, as long as more than half of the nodes in the random consensus community of $\mathcal{R}_i$ is benign. 

% \first Consistency for Honest Nodes. Since an honest sender will send the same $FC$ to all its community members in $\mathcal{R}_i$, all honest nodes will reach the same output. 

% \second Validity. If an honest sender correctly and reliably broadcasts $v$ in $\mathcal{R}_i$, then all honest nodes in the community will receive enough votes to accept it. Afterwards, all remaining honest nodes will eventually collect at least $f+1$ acceptance messages and accept $v$, after the second round of broadcast. 

% \third External-Validity. If a node reliably delivered $v$ in $\mathcal{R}_i$, then the node must have collected $f+1$ votes for $v$, and at least one of the votes is from an honest node in the community. Therefore, $v$ must be authentic (\ie it is a correctly constructed $FC$). 

% \subsection{BGP Validation}
% \label{sub:BGPValidation}
% $FC$s issued by honest ASes are correct and consistent with its BGP announcement, as guaranteed by our consensus protocols. However, since the malicious ASes can create arbitrary $FC$s on its behalf, it could either guide the community to reach consensus on a $FC$ inconsistent with real BGP announcements, or prevent the community from reaching consensus (for instance sending the $FC$ to only a small group of members). 
% Fortunately, these attacks do not impact \emph{end-to-end} path validation in \sys. In particular, in order to authenticate a BGP path, one AS needs to possess a confirmed $FC$ for every hop on the path. For instance, if the adversary wants to successfully manipulate the original path $\mathcal{P}{:} S {\leftarrow} A {\leftarrow} C {\leftarrow} E {\leftarrow} D$ to $\mathcal{P}{:} S {\leftarrow} A {\leftarrow} M {\leftarrow} D$ (where $M$ is an AS controlled by the adversary), the network needs to witness a valid $FC$ issued from AS $A$ to $M$ (\ie $\mathcal{F}_{\{A, M, \mathcal{P}\}}$), besides other $FC$s. Therefore, as long as AS $A$ is benign, the end-to-end path authentication would fail, even if $M$ can falsely claim a shortcut between $M$ and $D$ using a self-signed $FC$  $\mathcal{F}_{\{M, D, \mathcal{P}\}}$. Since \sys is designed based on the assumption that RoV is widely deployed (see \S~\ref{subsec:threat_model}), there exists at least one benign AS on the BGP path before the malicious AS $M$. Therefore, the end-to-end path authentication would never succeed. 

% \subsection{Forwarding Validation}
% \label{FV-analysis}
% \parab{Incorrect filtering table} Since the binding message will be signed by the source AS and the presence of RoV, it can be determined that the malicious AS cannot impersonate other ASes to issue verifiable binding messages. This means that there is no binding message generating an incorrect filter table that can affect the forwarding of legitimate traffic, only the possibility that the source AS binds its own traffic to the wrong path. In this case, the affected traffic is only the traffic declared in the binding message issued by the source AS. In addition, due to the wrong path, the source AS will soon detect that the traffic cannot be forwarded to the destination correctly (if it can reach the destination AS correctly, the binding information published by the source is still considered correct and valid), and will be able to troubleshoot the problem and re-publishing the binding message with an updated version number.

% \parab{Nodes without liveness} Although malicious nodes cannot spoof binding messages that can affect normal traffic, it is still possible for them to block legitimate binding messages, making some nodes inactive and never able to establish filter tables. However, we find that such an attack is difficult and makes the malicious node quickly exposed.

% First, binding messages use application layer broadcast to complete the synchronization between nodes. In the scenario of large throughput between domains, malicious nodes need to block specific traffic of specific nodes under specific applications (only binding messages are blocked, neighbor discovery or keep-alive messages are not blocked so that nodes are not automatically offline), and such filtering operation is very difficult. In addition, even if the malicious nodes can achieve efficient message interception, the quarantined node must be completely surrounded, which means that the path between the quarantined node and any other honest node must pass through the malicious nodes, then the quarantined node can find itself missing some of the latest binding messages after a consensus time slice and initiate the update operation. However, soon all update operations applied to surrounding neighboring nodes will time out, at which time the node can determine that it is under isolation attack and all directly connected neighboring AS are malicious nodes and can initiate out-of-band complaint and processing mechanism.

\subsection{Deployment}
\label{Deployment}

\parab{Slow Start in a Stable Network} 
In a well-established network, the number of new BGP updates is often much smaller than the total number of established BGP routes. For instance, the total number of BGP paths in the Caida dataset of Apirl 2023 is about 377 million. The number of BGP paths remain the same over the period of 4 months (from January 2023 to April 2023) is about 260 million, roughly  68.99\% of all paths.  
% of which the number of unchanged paths in 3 months is 166223084, 
Since new \fcs are generated only if BGP paths change, \sys may face a slow start issue that the  established BGP routes do not trigger \fcshort generation. Consequently, the subsequent data plane forwarding verification that relies on \fcshort binding relationships is also limited due to the lack of \fcs.  

% When a network already relies on BGP to establish rich links between ASes (such as the current Internet), and the entire network system is running steadily. This environment to deploy \sys additionally will face the challenge of a slow start-up. Because all BGP routes are not validated according to \sys, there is no $FC$ corresponding to the links, and the source cannot rely on the $FC$ list to specify the path. Waiting for route updates to gradually generate $FCs$ and initiate \sys would take a lot of time because BGP routes are not updated very frequently in a stable network system. More critically, for routes that have not been updated, the corresponding BGP path will never be included in the validation and protection of the \sys mechanism because of the lack of $FCs$.

As part of the initialization when an AS $N$ joins the \sys ecosystem, it shall generate an initial binding message for each of the local BGP routes. The version number $\textsf{Ver}$ in this message is set as a special indicator $0$, and the $\textsf{FC}_\textsf{list}$ is the inverse sequence of the AS-Path in the BGP route. The verification protocol of these messages are similar to regular the verification protocol (see \S~\ref{subsec:forward_binding}), except that no verification is needed for the  $\textsf{FC}_\textsf{list}$. 

% To address this issue, \sys has designed a fast-start deployment method that can quickly establish global authentication capability based on current routing information. For any AS $N$ that joins this mechanism, the corresponding initialization binding message is generated for all BGP routing entries of AS $N$. In the initialization binding message, 1) the version number $\textsf{Ver}$ is set to $0$. 2) the legitimate $\textsf{FC}_{list}$ is not available due to the lack of validation of the BGP announcement. In the initialization binding message with $\textsf{FC}_{list} = {0}$, the $\textsf{FC}_{list}$ is the inverse sequence of the AS-Path in the BGP route and is signed with the private key of the AS $N$.

% For the on-path node, validate the message signature and $FC$ list signature, check whether this AS is on the path, bind this traffic (source and destination prefixes) to the incoming port of this message after the check passes, and establish the filtering rule. For the off-path node, validate the message signature, confirm that this traffic does not pass through itself, and establish filtering rules.

The startup binding messages are also helpful to detect existing/established path manipulation or source spoof attacks. Suppose that from AS $S$'s perspective, its traffic $\langle \textsf{src}{:}S, \textsf{dst}{:}D\rangle$ expects to take the AS-path $S{\rightarrow}B{\rightarrow}C{\rightarrow}D$. Yet the actual forwarding path is manipulated as  $S{\rightarrow}M{\rightarrow}D$ to route through a compromised AS $M$. Once the traffic filters are constructed based on these startup messages, AS $D$ realize that traffic $\langle \textsf{src}{:}S, \textsf{dst}{:}D\rangle$ received from $M$ is unauthorized, and therefore should be discarded. 
Similarly, ASes can discard spoofed traffic based on these startup binding messages. 

% Relying on the above operation, \sys can be quickly started globally according to the BGP routing information currently in use, and the corresponding filtering rules can be established. After the initial filtering mechanism is established, the authenticity of the BGP routing information currently in use can be validated, and cases where the actual forwarding path is inconsistent with the BPG announcement can be discovered, and various attacks caused by this can be effectively detected. For example, the case where traffic is hijacked by forging an AS-path that is shorter than the actual path, but still provides connectivity between the source and destination. Since the path specified by the source (the fake AS-Path) does not match the actual forwarding path, the unauthorized nodes on the fake path will not receive the on-path binding message from the source, and being an off-path node, the relevant traffic will be dropped and the connection between the source and the destination will be broken, so the attack will be detected by source AS. Similarly, malicious traffic that tampers with the forwarding path or spoofs the source address will also be filtered.

\parab{Initial Network} 
Contrary to the stable/established network is a newborn network without full connectivity yet. Thus, it is possible that some AS pairs do not have viable paths between them. %violating the second assumption in \S~\ref{subsec:threat_model}. 
To facilitate startup in a newborn network, we can rely on several well-connected service providers or CDNs to relay binding messages ASes. Specifically, instead of direct message broadcast, ASes can adopt a pub-sub mechanism to publish and pull binding messages from these service providers. 
Once the initialization phase is complete, \sys can switch back to the normal operation mode. 

\iffalse 
When a network is in the initialization phase, there may not be available routing paths between each AS at this time. IP reachability between all AS cannot be guaranteed, the assumption 2 in \S~\ref{subsec:threat_model} %~\ref{sec:consensus_SIG23} 
is not satisfied. 
For the network initialization situation, \sys designs an alternative startup scheme. \sys will set up several TOP service providers (such as Google, Amazon, Microsoft, etc.) accessible by all nodes to provide network bulletin board services, in order to provide the necessary inter-node connectivity guarantees for the network initialization phase. The following assumptions need to be satisfied at this point.

Assumption 1: The link between any node and the service provider is not dependent on other service providers.

Assumption 2: For all selected service providers, at least one of them is honest and reliable.

For any AS $N$, BGP announcement and validation will be performed according to \sys, and a binding message will be generated based on the validated BGP announcement. After that, AS $N$ will send the binding message to all selected service providers. Any other AS $M$, which will subscribe to all service providers, will generate the local filtering table based on the binding message obtained from any service provider record after the signature validation is passed.
For the following reasons, we propose to switch back to consensus and broadcast when the initialization phase is completed, that means IP reachability between nodes can be guaranteed, for the following reasons:

1) This will rely on a more centralized infrastructure.

2) Overly concentrated network bandwidth pressure.

3) More end-to-end transmissions, resulting in wasted resources (1-time end-to-end communication becomes 2 times end-to-end communications between ASes to service providers)
\fi

==> overview.tex <==
\section{Overview}

\subsection{Design Goals}
\label{subsec:design_goals}

\parab{Compatibility and Incremental Deployability} We prefer to not profoundly change the status-quo of the inter-domain routing protocol (\ie BGP) in the Internet. Meanwhile, due to different levels of sophistication and scale, we do not expect all ASes will simultaneously upgrade their routing/forwarding devices to support \sys. 
Therefore, the primary design goal of \sys is to be compatible with the current BGP inter-domain routing protocol. Meanwhile, \sys should be incrementally deployable (\ie an AS can receive deployment benefits without depending on whether other ASes  deploy \sys or not), avoiding the dilemma of deployment motivation (\ie the chicken-and-egg problem~\cite{2011Mirage}).  

% it can provide instant benefits to the first adopter. not require complete deployment to be effective. 

% \sys should not introduce significant modifications to existing protocols or network equipment, using existing Internet infrastructure and extensions to existing protocols to achieve this. At the same time, \sys needs to support partial deployments, while monotonic deployment benefits can be obtained.

\parab{Security Goals} \sys is designed to enhance the security of control plane routing and dataplane forwarding in the Internet at the network layer. Specifically, \sys allows an AS to independently prove its BGP routing decisions with publicly verifiable cryptography commitments, based on which any on-path AS can verify the authenticity of a BGP path; meanwhile \sys ensures the consistency between the control plane and dataplane, \ie the network traffic must take the forwarding path that is consistent with the control plane routing decisions, or otherwise being discarded.   
More crucially, the above security guarantees offered by \sys are not binary, \ie secure or non-secure. Instead, the security benefits (quantifiable using multiple metrics in \S~\ref{sub:SecurityBenefits}) are strictly monotonically increasing as the deployment rate of \sys (\ie the percentage of ASes that are upgraded to support \sys) increases. 
The security of other layers (\eg the application layer) is out of scope. 
% The security goal of \sys is to enhance the control-plane and data-plane security in the Internet. %the network layer, providing the ability to verify behavior consistency across planes. 
% Control-plane security refers to the ability to enhance the authenticity assurance of AS paths in BGP update messages. Data-plane security refers to guaranteeing that traffic comes from the real source and is correctly forwarded according to the path announced by the route. 
% For guaranteeing the authenticity of packet payload is out of the scope of this paper.

\parab{Lightweight} 
To avoid significant overhead, \sys adopts a per-hop verification scheme for validating BGP updates. Considering that most of the Internet BGP updates are partial updates of BGP paths, such a design helps to significantly reduce the validation overhead (see \S\ref{subsubsection:Internet Validation} for more details).
%This lowers the worst-case cryptographic overhead from $O(N^2)$, as in BGPsec, to $O(N)$, where $N$ is the number of hops. Crucially, the concrete verification overhead is often much smaller than $O(N)$, because only the changed hops on a BGP path need to be re-verified. 
On ensuring that only authenticated inter-domain paths are used for dataplane forwarding, \sys can employ the readily available ACL filters on hardware routers to discard unwanted traffic at line-speed. 

\subsection{Threat Model and Assumptions}
\label{subsec:threat_model}

% On control plane of Internet inter-domain routing, we consider that BGP source hijacking and AS-path manipulation are two orthogonal attacks. 

We assume that ASes participating in \sys have access to an Internet-scale trust base, namely Resource Public Key Infrastructure (RPKI), that stores authoritative information about the mapping between AS numbers and their owned IP prefixes, as well as ASes' public keys. 

% \textit{Assumption 1:} All joining ASes have RPKI-like source verification capability, the legal mapping between AS number, legal IP prefixes and AS public key can be globally verified (Combination of end entity (EE) certificates issued under a RPKI Certification Authority (CA) certificate of an AS, such as ROAs and router certifications). Further, we do not consider the case where two colluding malicious ASes manipulate the hop between them. For instance, changing the path for prefix $\mathcal{P}$ from $\mathcal{P}{:}A {\leftarrow} B {\leftarrow} D$ to $\mathcal{P}{:}A {\leftarrow} B {\leftarrow} C {\leftarrow} D$ where $B$ and $C$ are colluding ASes. 

%\textit{Assumption 2:} IP reachable between all joining AS. The cases in which this assumption cannot be met are discussed in the section~\ref{sec:analysis}. \sys relies on a distributed consensus protocol to build a global view on cross-planes consistency. To ensure the correctness of consensus, we model the network as an Stable Internet Routing system~\cite{gao2001stable}. Specifically, we assume that \first The network graph of honest nodes is well connected. \second The communication channels between honest nodes are asynchronous~\cite{gao2001stable,miller2016honey,duan2018beat}.


Given above assumptions, we consider the following adversary. \first On the control plane, the adversary can launch \emph{path manipulation attacks}. 
This means that the adversary will try to manipulate the routing paths to victim ASes or prefixes by sending bogus BGP updates. For example, the adversary might try to reroute traffic to the victim ASes/prefixes through ASes that they control, in order to perform (encrypted) traffic analysis.
% Note that we do not consider the case where two colluding malicious ASes manipulate the hop between them since the two colluding ASes are can virtually considered 
\second On the dataplane, the adversary can spoof source addresses and send unwanted network traffic to the victim ASes/prefixes. 



% \first An adversarial AS can eavesdrop the BGP announcements from all its neighbors. \second It may issue false route announcements to the victim prefix to the surrounding neighbors. \second The attacker can manipulate the forwarding of traffic flowing through (as compared to the control-plane announcement path). \third The attacker can send spoofed source address packets. Attacker can spoof the legitimate prefix of any victim AS to send a spoofed source address packet.

% As an attacker cannot lie about its AS number, the fake route announcement will carry the AS-path starting from the victim AS and ending with the attacker. The attacker cannot launch prefix or sub-prefix attacks due to the existence of RoV, and will launch n-hop route path tampering attacks.



% \begin{figure}
%  \includegraphics[width=0.45\textwidth]{BGP-Latex/picture/General8.pdf}
%  \caption{Overview of \sys.}
% \label{FC}
% \end{figure}


\subsection{Building Blocks} 
\parab{Forwarding Commitment} \sys enhances the security of inter-domain routing and forwarding by building a publicly verifiable view on \emph{forwarding commitments}. At a high-level, a routing commitment (\fcshort) of an AS is a cryptographically-signed primitive that binds the AS's routing decisions (\eg willing to forward traffic for a prefix via a certain hop). With this view, ASes are able to \first evaluate the authenticity (or security) of the control plane BGP announcements based on committed routing decisions from relevant ASes, and \second ensure that the data plane forwarding is consistent with the routing decisions committed in the control plane. 

% In particular, with this view, each AS is able to \first make public commitments to the entire network regarding its BGP routing decisions and forwarding paths (\eg willing to forward traffic for a prefix on a certain BGP path), \second 

% \sys employs a distributed consensus protocol, optimized based on BGP semantics, to ensure that the entire network reaches consensus on a single view of traffic and routing path binding relationships. Crucially, such a publicly verifiable view does not undermine the BGP privacy, \ie it does not reveal AS topology relationships and AS routing preferences or polices. 



% and briefly describe how \sys performs BGP path validation on the control plane, forwarding validation on the data plane, and consistency assurance between the two planes via $FC$s.




\parab{BGP Path Validation} Consider an illustrative example using the four-AS topology shown in Figure~\ref{example}. 
% In this process, \sys generates the corresponding $FC$ and adds it to the community field of the BGP announcement so that the receiving AS can validate the authenticity of the announcement. 
Suppose AS $C$ receives a BGP announcement $\mathcal{P}_A{:}A {\leftarrow} B {\leftarrow} C$ from its neighbor $B$. If AS $C$ decides to further advertise this path to its neighbor $D$ based on its routing policy, it generates a \fcshort $\mathcal{F}_{\{C,D,\mathcal{P}\}}$, adds it to the community field of the BGP announcement, and forwards the BGP update message to $D$. 
% publicly commit its routing decision to the AS $D$. 
When AS $D$ receives the route from $C$, it can determine the authenticity of the current AS path by verifying the list of \fcs carried in the BGP announcement correctly reflects the AS path. The exact computation of $\mathcal{F}_{\{C,D,\mathcal{P}\}}$ is explained in \S~\ref{subsec:fc_design}. 


% including four ASes $A$, $B$, $C$, $D$. 
% We propose Forwarding Commitments ($FC$) to construct such publicly verifiable views. As shown in Figure~\ref{FC}, when AS A announces a BGP route to AS B, it will also generate a corresponding $FC$, based on which the AS B can verify the authenticity of the received route announcement. AS B can then bind specific traffic to this $FC$, and AS A uses this binding relationship to verify the receiving traffic. 

% AS $A$ announces the BGP route reaching prefix $\mathcal{P}_A$ to AS $B$, AS $B$ announces it to AS $C$, and AS $C$ announces it to AS $D$. 


\parab{Forwarding Validation} To enable forwarding validation, ASes need to announce the traffic-\fcs binding relationship. Specifically, suppose AS $D$ confirms that the AS-path $C{\rightarrow}B{\rightarrow}A$ reaching $\mathcal{P}_A$ is legitimate, it binds the traffic $\langle \textsf{src}{:}\mathcal{P}_D, \textsf{dst}{:}\mathcal{P} \rangle$ (where $\mathcal{P}_D$ is the source prefix owned by AS $D$) with the \fcshort list $\{ \mathcal{F}_{\{C,D,\mathcal{P}\}};\mathcal{F}_{\{B,C,\mathcal{P}\}};\mathcal{F}_{\{A,B,\mathcal{P}\}} \}$, and then publicly announces the binding relationship. 
Upon receiving the relationship, other ASes can build traffic filtering rules to enable path validation. For instance, by interpreting the binding relationship produced by AS $D$, AS $C$ confirms that the traffic $\langle \textsf{src}{:} \mathcal{P}_D, \textsf{dst}{:}\mathcal{P}_A \rangle$ shall be forwarded on link $L_{CD}$, and AS $B$ confirms that the traffic shall be forwarded on link $L_{BC}$. 
Network traffic violating these binding rules are not legitimate. 

To enable network-wide forwarding verification, these binding rules are broadcast globally (instead of just informing the ASes on the AS-path) so that off-path ASes can also discard unauthorized flows. We design a lightweight protocol, optimized using BGP semantics, to achieve fast binding relationship synchronization globally. 

% After the route to prefix $\mathcal{P}_A$ is validated, AS $B$, $C$, and $D$ \emph{binds} the network traffic to $\mathcal{P}_A$ to the corresponding \fcshort list, by publicly announcing the committed forwarding path for the traffic to the entire network. Based on this binding relationship, other ASes build traffic filtering tables to validate the packets' forwarding path and source authenticity, ensure data-plane and control-plane consistency. 

% For example, after AS D confirms that route $C{\rightarrow}B{\rightarrow}A$ to $\mathcal{P}_A$, AS D binds traffic with its own prefix as the source address and $\mathcal{P}_A$ as destination address, to path $C{\rightarrow}B{\rightarrow}A$, corresponding to $\mathcal{F}_{\{C,D,\mathcal{P}\}}-\mathcal{F}_{\{B,C,\mathcal{P}\}}-\mathcal{F}_{\{A,B,\mathcal{P}\}}$, and announces this binding relationship to the entire network in a privacy-protected way. 

% Other ASes received this binding message can build a checking table to filter the traffic that is off the path, but claims to be from AS $D$ to $\mathcal{P}_A$ to ensure data-plane forwarding and control-plane consistency. Afterwards, the whole network is informed of the binding relationship through a broadcasting and distributed consensus protocol described in \S~\ref{sec:consensus_SIG23}. 
